A Private and Computationally-Efficient Estimator for Unbounded Gaussians

We give the first polynomial-time, polynomial-sample, differentially private estimator for the mean and covariance of an arbitrary Gaussian distribution $\mathcal{N}(\mu,\Sigma)$ in $\mathbb{R}^d$. All previous estimators are either nonconstructive, with unbounded running time, or require the user to specify a priori bounds on the parameters $\mu$ and $\Sigma$. The primary new technical tool in our algorithm is a new differentially private preconditioner that takes samples from an arbitrary Gaussian $\mathcal{N}(0,\Sigma)$ and returns a matrix $A$ such that $A \Sigma A^T$ has constant condition number.

==> ballfinder.tex <==
\section{Ball Finding Algorithm}

\begin{algorithm}[h!] \label{alg:ballfinder}
\caption{Naive Private Ball Finder
    $\ballfinder_{\eps, \delta, \beta, R}(X)$}
\KwIn{A set of $n$ samples $X_1, \dots, X_n \in \RR^{D}$ from an unknown Gaussian.
    Parameters $\eps, \delta, \beta, R > 0$}
\KwOut{A point $c \in \RR^{D}$.}
\vspace{10pt}

Set parameter: $\ell \gets \tfrac{R}{100\sqrt{D}}$
\vspace{10pt}

Discretize $\RR^D$ into $\Omega \gets \{i\ell : i \in \Z\}^D$.\\
Round each $X_j$ to the nearest grid point in $\Omega$ to get $Y_j$.\\
Let $Y \gets (Y_1,\dots,Y_n)$.\\
Set $c \gets \goodcenter_{\eps,\delta,\beta,\Omega,R}(Y)$.
\vspace{10pt}

\Return $c$
\vspace{5pt}
\end{algorithm}

\begin{thm}[$\goodcenter$ from \cite{NissimS18}]\label{thm:goodcenter}
\end{thm}

\begin{thm}\label{thm:ballfinder}
\end{thm}


==> covariance-old.tex <==
\section{Estimating Covariance of Gaussians}

\begin{algorithm}[h!]
\label{alg:dpgce}
\caption{DP Gaussian Covariance Estimator
    $\DPGCE_{\eps, \delta, \alpha, \beta}(X)$}
\KwIn{Samples $X_1,\dots,X_{n} \in \R^d$.
    Parameters $\eps, \delta, \alpha, \beta > 0$.}
\KwOut{Projection matrix $\wh{\Pi} \in \R^{d \times d}$ of rank $k$.}
\vspace{5pt}

Split $X$ into datasets of size $\lfloor n/2 \rfloor$: $Y,Z$.
\vspace{5pt}

\tcp{Estimate the eigenvalues of the covariance.}
$(\hat{\lambda}_1,\dots,\hat{\lambda}_d) \gets
    \DPEE_{\frac{\eps}{2},\frac{\delta}{2},\frac{\beta}{2}}(Y)$.\\
\vspace{5pt}

\tcp{Return the estimate.}
\Return $\DPRGCE_{\eps,\delta,\alpha,\beta,d}(Z,\hat{\lambda}_1,\dots,\hat{\lambda}_d).$
\vspace{5pt}
\end{algorithm}

\begin{algorithm}[h!]
\label{alg:dprgce}
\caption{DP Recursive Gaussian Covariance Estimator
    $\DPRGCE_{\eps, \delta, \alpha, \beta, d}(X,\hat{\lambda}_1,\dots,\hat{\lambda}_k)$}
\KwIn{Samples $X_1,\dots,X_{m} \in \R^d$.
    Eigenvalues $\hat{\lambda}_1,\dots,\hat{\lambda}_k$.
    Parameters $\eps, \delta, \alpha, \beta > 0$.}
\KwOut{Projection matrix $\wh{\Pi} \in \R^{d \times d}$ of rank $k$.}
\vspace{5pt}

Set parameters:
    $\gamma^2 \gets C_2\cdot SOMETHING$
    \qquad $\eps' \gets \tfrac{k\eps}{d}$
    \qquad $\delta' \gets \tfrac{k\delta}{d}$
    \qquad $\beta' \gets \tfrac{k\beta}{d}$
\vspace{5pt}

\tcp{If condition number is small, we can use the learner from $\KLSU$.}
\If{$\hat{\kappa} \leq 16\cdot2^d$}{
    \Return $\KLSU_{\eps',\delta',\alpha,\beta'}(X)$.
}
\vspace{5pt}

\tcp{Find large eigenvalue gap to project on to low dimensional subspace.}
Let $r$ be the smallest number, such that
    $\tfrac{\hat{\lambda}_r}{\hat{\lambda}_{r+1}} > \gamma^2$.\\
$\Pi_r \gets \subspace_{\eps',\delta',
    \beta',\frac{\alpha}{16\cdot\kappa kd^{2}}}$,
    and $\Pi_{k-r}$ be the orthogonal projector of $\Pi_r$.
\vspace{5pt}

\tcp{Recurse on the lower dimensional subspaces.}
Partition $X$ into $X^1$ of size $\tfrac{rm}{k}$ and
    $X^2$ of size $\tfrac{(k-r)m}{k}$.\\
\Return $\DPRGCE_{\eps,\delta,\alpha,\beta,d}(\Pi_r X^1,\hat{\lambda}_1,\dots,\hat{\lambda}_r) +
    \DPRGCE_{\eps,\delta,\alpha,\beta,d}(\Pi_{k-r} X^2,\hat{\lambda}_{r+1},\dots,\hat{\lambda}_k)$
\vspace{5pt}
\end{algorithm}


==> stupid.tex <==
\section{Closing the Gap}

Suppose the private data $x_1, \cdots, x_n \in \mathbb{R}^d$ consists of $n$ independent draws from $N(0,\Sigma)$ with $\Sigma = U \Lambda U^T$ and $U, \Lambda, \Sigma \in \mathbb{R}^{d \times d}$, where $U^TU=I$ and $\Lambda$ is diagonal with entries $\lambda_1 \ge \lambda_2 \ge \cdots \ge \lambda_d \ge 0$.

Using a subsample and aggregate method with a histogram algorithm, we can privately estimate the eigenvalues. Thus we have $\tilde\lambda_1 \ge \tilde\lambda_2 \ge \cdots \tilde\lambda_d \ge 0$ with $(1-\tau)\lambda_i \le \tilde\lambda_i \le (1+\tau) \lambda_i$ for all $i$, where $\tau>0$ is some accuracy parameter.

Let us assume that there is a large eigengap -- i.e., $\lambda_{k+1} \le \gamma \cdot \lambda_k$ for some $k \in [d]$ and $0 < \gamma \ll 1$. We then run the subspace algorithm \cite{SinghalS21} to obtain $\tilde{U} \in \mathbb{R}^{d \times d}$ satisfying $\tilde{U}^T\tilde{U}=I$ and $\|\tilde{U}_{1:k}\tilde{U}_{1:k}^T - U_{1:k}U_{1:k}^T\| \le \alpha$. Here $U_{1:k} \in \mathbb{R}^{d \times k}$ denotes matrix consisting of the first through $k$-th columns of $U \in \mathbb{R}^{d \times d}$.

Now let $y_i = (I-\eta \tilde{U}_{1:k}\tilde{U}_{1:k}^T) x_i$ for all $i \in [n]$. Here $0 \le \eta < 1$. Then $y_1, \cdots, y_n \in \mathbb{R}^d$ are $n$ independent draws from $N(0,\hat\Sigma)$, where \[\hat\Sigma = (I-\eta \tilde{U}_{1:k}\tilde{U}_{1:k}^T) \Sigma (I-\eta \tilde{U}_{1:k}\tilde{U}_{1:k}^T)^T.\]

Now, if we can learn $\hat\Sigma$ from $y_1, \cdots, y_n$, we can learn $\Sigma$ from $x_1, \cdots, x_n$. The goal of this reduction is close the eigenvalue gap. That is, the eigenvalues of $\hat\Sigma$ shouldn't have the same gap that those of $\Sigma$ have. It remains to carefully calculate the relationship between the two sets of eigenvalues.

We have
\begin{align*}
    \hat\Sigma &= (I-\eta \tilde{U}_{1:k}\tilde{U}_{1:k}^T) \Sigma (I-\eta \tilde{U}_{1:k}\tilde{U}_{1:k}^T)^T\\
    &= (I - \eta U_{1:k} U_{1:k}^T - \eta (\tilde{U}_{1:k} \tilde{U}_{1:k}^T - U_{1:k} U_{1:k}^T)) U \Lambda U^T (I - \eta U_{1:k} U_{1:k}^T - \eta (\tilde{U}_{1:k} \tilde{U}_{1:k}^T - U_{1:k} U_{1:k}^T))^T\\
    &= (I - \eta U_{1:k} U_{1:k}^T - \xi) U \Lambda U^T (I - \eta U_{1:k} U_{1:k}^T - \xi)^T\\
    &= ((1-\eta) U_{1:k} U_{1:k}^T + U_{k+1:d}U_{k+1:d}^T- \xi) (U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T) ((1-\eta) U_{1:k} U_{1:k}^T + U_{k+1:d}U_{k+1:d}^T- \xi)^T\\
    &= (1-\eta)^2 U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T \\ &~~~ - \xi (U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T) ((1-\eta) U_{1:k} U_{1:k}^T + U_{k+1:d}U_{k+1:d}^T)^T \\ &~~~ - ((1-\eta) U_{1:k} U_{1:k}^T + U_{k+1:d}U_{k+1:d}^T ) (U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T) \xi^T \\ &~~~ + \xi (U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T) \xi^T \\
    &= (1-\eta)^2 U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T \\ &~~~ - \xi ((1-\eta) U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T)  \\ &~~~ -  ((1-\eta) U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T) \xi^T \\ &~~~ + \xi (U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T) \xi^T,
\end{align*}
where $\xi = \eta (\tilde{U}_{1:k} \tilde{U}_{1:k}^T - U_{1:k} U_{1:k}^T)$. We have $\|\xi\| \le \alpha$.

Let $\overline\Sigma = (1-\eta)^2 U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T$. Then
\begin{align*}
    \| \hat\Sigma-\overline\Sigma\| &\le 2 \|\xi\|\cdot  \| (1-\eta) U_{1:k} \Lambda_{1:k} U_{1:k}^T + U_{k+1:d} \Lambda_{k+1:d} U_{k+1:d}^T \| + \|\xi\|^2 \cdot \|\Sigma\| \\
    &\le 2 \|\xi\| ((1-\eta) \lambda_1 + \lambda_{k+1}) + \|\xi\|^2 \lambda_1\\
    &\le \alpha(2(1-\eta)+\alpha)\lambda_1 + 2\alpha \lambda_{k+1}.
\end{align*}

The last todo is to see if the parameters work out. For simplicity, assume $\lambda_1 \approx \lambda_k$ and $\lambda_{k+1} \approx \lambda_d$ -- i.e., there is only the one large gap between $\lambda_k$ and $\lambda_{k+1}$. Then we want to set $\eta$ such that $(1-\eta)^2 \lambda_k \approx \lambda_{k+1}$. This would ensure that there are no large gaps in $\overline\Sigma$. If $\|\hat\Sigma-\overline\Sigma\| \ll \lambda_{k+1}$, then this ensures that there are no large gaps in $\hat\Sigma$, as desired. We have $\|\hat\Sigma-\overline\Sigma\| \le O(\alpha \cdot \sqrt{\lambda_{k+1}\lambda_k})$. Thus we require $\alpha \ll \sqrt{\lambda_k/\lambda_{k+1}} \approx \sqrt{\gamma}$.

The results of Singhal and Steinke \cite{SinghalS21} give \[\alpha = O\left(\gamma \cdot \frac{d k^{1.5} \sqrt{\log(1/\delta)\cdot (k + \log(k \log(1/\delta)/\varepsilon)}}{\sqrt{\varepsilon n}}\right).\]

This seems like it would work as long as $\gamma$ is sufficiently small. Specifically, if $\gamma \ll \frac{\varepsilon n}{d^2 k^3 {\log(1/\delta)}\cdot (k + \log(k \log(1/\delta)/\varepsilon)}$, then the above works out.
